Differentiable Submodular Maximization

We consider learning of submodular functions from data. These functions are important in machine learning and have a wide range of applications, e.g. data summarization, feature selection and active learning. Despite their combinatorial nature, submodular functions can be maximized approximately with strong theoretical guarantees in polynomial time. Typically, learning the submodular function and optimization of that function are treated separately, i.e. the function is first learned using a proxy objective and subsequently maximized. In contrast, we show how to perform learning and optimization jointly. By interpreting the output of greedy maximization algorithms as distributions over sequences of items and smoothening these distributions, we obtain a differentiable objective. In this way, we can differentiate through the maximization algorithms and optimize the model to work well with the optimization algorithm. We theoretically characterize the error made by our approach, yielding insights into the tradeoff of smoothness and accuracy. We demonstrate the effectiveness of our approach for jointly learning and optimizing on synthetic maximum cut data, and on real world applications such as product recommendation and image collection summarization.

==> experiments_no_dpp.tex <==
%!TEX root = main.tex

\section{Experiments}
\label{sec:experiments}

\subsection{Maximum Cut}
Let $G(V, E, w)$ be a weighted undirected graph, where $V$ denotes the set of vertices, $E$ is the set of edges and $w$ denotes the set of non-negative edge weights $w_{ij}$, $\forall (i,j) \in E$. The maximum cut problem is to find a subset of nodes $S$ such that the cut value $f(S) = \sum_{i \in S} \sum_{j \in V \setminus S} w_{ij} $ is maximized. The cut function $f(S)$ is a non-negative and non-monotone submodular function and has, for instance, been used in semi-supervised learning~\cite{maxcutsemisupervised}. 

\noindent We generate synthetic data for our maximum cut experiment as follows. We first generate $n$ vectors $x_1, \ldots, x_n$ whose components are sampled from $\mathcal{U} {\sim} (0,1)$ in $\mathbb{R}^d$ and arrange them in a $n \times d$ matrix $\mathbf{X}$. Using a projection matrix $\mathbf{P}$, we project each $x_i$ to the lower dimensional space $\mathbb{R}^k$. The weights of the graph $w$ are generated using an RBF kernel $\mathbf{K}$ on these transformed points. For the resulting graph instance $G(V, E, w)$ we compute the maximum cut $S^{*} \subseteq V$ using MIP (Mixed Integer Programming).

\noindent We sample $\mathbf{X}_1, \mathbf{X}_2, \ldots, \mathbf{X}_m$ as described above and, using the $\textit{same}$ projection matrix $\mathbf{P}$ and RBF kernel $\mathbf{K}$, we generate weights $w^{i}$ for $m$ graphs and find the maximum cut $S^{*}_{i}$ by MIP for each of these graphs. From this data we compose our training set as $\mathcal{X}=\{ (\mathbf{X}_1, S^{*}_{1}), \ldots, (\mathbf{X}_m, S^{*}_{m})\}$. The test set is composed using the same strategy. 

\noindent In this experiment, our aim is to learn a projection matrix  $\hat{\mathbf{P}}$ such that \alg, if executed on the graph induced by the points $\hat{\mathbf{P}} \mathbf{X}_i$, returns $S^{*}_i$. Note that our goal is not necessarily to recover the original projection matrix $\mathbf{P}$---we are only interested in a projection matrix that allows us to find high value cuts through \alg.
For each element of the test set, we compute the corresponding graph using $\hat{\mathbf{P}}$ and find the maximum cut using  \alg and call the set as $S^{l}_{DG}$. We compute the corresponding graph using $\mathbf{P}$  and a random projection matrix, which acts as a baseline, $\mathbf{P}_{r}$ and find the maxcut using \alg; we refer to these cuts as $S^{o}_{DG}$ and $S^{r}_{DG}$  respectively. When the cut value is calculated using MIP, we call it as $S^{o}_{MIP}$. We compare the ratio of the each cut value calculated by \alg to the cut value calculated by MIP.

\noindent Results are shown in Table~\ref{tab:maxcut}. We observe that cuts computed with \alg using the learned projection matrix outperform cuts computed via random projection matrices and the original projection matrix. The number of nodes in the graph is $n$, the temperature of the  \alg is $t$ and $0.3$ is used as a bandwith parameter for the RBF kernel. The original points $x_i$ are in $\mathbb{R}^{10}$ and they are projected into $\mathbb{R}^5$ using the first 5 coordinates. Our training and test set consists of $800$ and $200$ elements, respectively. During training and testing, we used $g_4(a,b;t)$ to define the likelihood of sets as in Equation~\eqref{eq:ll}. For optimization, we used Adam~\cite{kingma2014adam} with batch size of $20$ and initial learning rate $0.01$. In every case, we benefit from learning the projection matrix.
%The original and the learned projection matrices are illustrated in the Appendix. %Moreover, Figure~\ref{fig:figure1} illustrates that learned matrix captures the subspace spanned by the original matrix. 

\input{table_maxcut.tex}

%\begin{figure}[h!]
%   \begin{subfigure}[b]{.5\linewidth}
%     \centering
%     \includegraphics[width=0.8\textwidth]{original}
%  	  \caption{Original projection matrix}
%	\end{subfigure}%
%   \begin{subfigure}[b]{.5\linewidth}
%     \centering
%     \includegraphics[width=0.8\textwidth]{learned}
%	  \caption{Learned projection matrix}
%   \end{subfigure}
%   \caption{(a) Original projection matrix and (b) learned projection matrix using \alg.}
%   	\label{fig:figure1}
%\end{figure}
%
%\textcolor{red}{Insert Plots}
%
%\subsection{Ordering of items in \alg}



%\textcolor{red}{Add Table and matrix}

\subsection{Product recommendation}

We consider the Amazon baby registry data~\cite{gillenwater2014em}.
%, initially used to train DPPs from data using an EM type procedure~\cite{gillenwater2014em}.
 The data consists of baby registry data collected from Amazon and split into several datasets according 
to product categories, e.g.\ safety, strollers, etc. The datasets contain $5{,}500$ to $13{,}300$ registries of users. The data is processed using 10-fold cross-validation. As for \alg the order of items matters, we permute the items according to their empirical frequencies  for each dataset. % in the training data
% More details can be found in~\cite{gillenwater2014em,tschiatschek2016learning}.

\noindent For every dataset and fold, we fit a facility location diversity (FLID) type model~\cite{tschiatschek2016learning}, i.e.
\begin{equation*}
  f(S) = \sum_{i \in S} u_i + \underbrace{\sum_{d=1}^D \big( \max_{i \in S} w_{i,d} - \sum_{i \in S} w_{i,d}\big)}_{\textnormal{div}(S)},
\end{equation*}
where $u_i \in \mathbb{R}$ encodes the utility of product $i$ and $w_{i,d} \in \mathbb{R}_{\geq 0}$ encodes the $d$th latent property of item $i$. The intuitive idea behind the term $\textnormal{div}(S)$ is to encode repulsive dependencies between items that all have the $d$th latent property.

\noindent We train FLID models by optimizing the likelihood of the training data in Equation~\eqref{eq:ll} for $t=1$ and the random approximation (\FLIDD) and by optimizing the likelihood in Equation~\eqref{eq:ll-greedy} (\FLIDG) for $t=10$. For optimization we uses stochastic gradient descent with a batch size of $1$ for \FLIDD{} and Adam with a batch size of $100$ for \FLIDG. We decayed the initial learning rate of $0.1$ with a decay factor of $0.9$ per epoch. We trained all models for 20 epochs.
%(iteration over all registries of a specific dataset).
The number of latent dimensions $D$ is $10$ for ground sets with up to 40 items and $20$ for larger ground sets.

\noindent {\bfseries Performance evaluation.} To assess the performance of our trained models we compute the following performance measures and compare them to the performance of \emph{modular} models (fully factorized models independently predicting the inclusion of any element in a set without considering correlations).
% and determinantal point process (DPPs) fitted by expectation maximization~\cite{gillenwater2014em}.
Let $\D=\{ R_1, \ldots, R_N\}$ be a set of registries and let $\bar{\D}=\{ R \in \D \mid |R| > 1\}$ be the set of registries in $\D$ with at least 2 items.
\begin{itemize}
  \itemsep0em 
  \item \emph{Relative improvement in likelihood \llgain.} This measure quantifies the  increase in likelihood for FLID over a modular model. The \llgain is computed as
    \begin{equation*}
      \llgain  = \frac{|\sum_{R \in \D} \log P(R) - \textnormal{LL}_\textnormal{mod}|}{\textnormal{LL}_\textnormal{mod}},
    \end{equation*}
    where $P(R)$ is the probability of $R$ for FLID and $\textnormal{LL}_\textnormal{mod} = \sum_{R \in \D} \log P_{\textnormal{modular}}(R) \log$ is the likelihood of the fully factorized model.
  
  \item \emph{Fill-in accuracy \Acc.} We test how accurately the considered models can predict items removed from a baby registry.  We compute the fill-in accuracy as
    \begin{equation*}
      \Acc(\D; \hat{f}) = \frac{1}{|\bar{\D}|} \sum_{R=\{ r_1, \ldots, r_k \} \in \bar{\D}} \sum_{i=1}^k \mathbf{1}_{\hat{f}(R - {r_i}) = r_i}
    \end{equation*}
    where $\hat{f}$ is the function used for prediction. For FLID and modular functions, $\hat{f}(S) = \arg \max_{e \in \groundset \setminus S} P(S + e)$.
    % In the case of DPPs, $\hat{f}$ returns the element with largest marginal conditioned on $S$.
    
  \item \emph{Mean reciprocal rank \MRR.} Instead of only accounting correct predictions, this measure considers the order in which the models would predict items. Formally, \MRR is defined as
    \begin{equation*}
      \MRR(\D; \hat{f}) = \frac{1}{|\bar{\D}|} \sum_{R=\{ r_1, \ldots, r_k \} \in \bar{\D}} \sum_{i=1}^k \frac{1}{r(r_i;R - {r_i})},
    \end{equation*}  
    where $r(r_i; R-r_i)=k$ if the item $r_i$ would be predicted as the $k$th item. % Thus \MRR can be seen as a smoothened version \Acc.

\end{itemize}


\noindent The results are shown in Table~\ref{tab:amazon}. We observe that FLID in most cases significantly outperforms the modular model in terms of fill-in accuracy and MRR. Furthermore, in the case of \FLIDD{}, we observe improved likelihood compared to the modular model.
%In many cases (for small ground sets) it also outperforms DPPs in terms of fill-in accuracy and MRR, while it performs similarly for larger ground sets. This findings are consistent with those in~\cite{tschiatschek2016learning}, where FLID was trained using noise-contrastive estimation (NCE). The application of NCE requires the definition of a noise distribution and the generation of noise samples which can be difficult for challenging dependencies in the data.
%Additionally, learning FLID using NCE yields only an approximately normalized model, rendering the computation of exact likelihoods difficult.

\input{table_amazon.tex}

%{\bfseries Computational complexity.}

%\textbf{Learning from product descriptions}

%\subsection{Image collection summarization}
%
%We consider the problem of image collection summarization, i.e.\ the problem of selecting a subset of images $S$ of an image collection $\groundset$ such that the selected images summarize the content of the collection $\groundset$ well (e.g.\ $S$ covers all important scenes in $\groundset$ and the pictures in $S$ are diverse).
%
%\noindent {\bfseries Data.} 
%We use the image collection summarization data from~\cite{tschiatschek2014learning}. 
%This data consists of 14 image collections $\groundset_1, \ldots, \groundset_{14}$, each  consisting of 100 images, i.e.\ $\groundset_i = \{ I^{(i)}_1, \ldots, I^{(i)}_{100} \}$.
%The images capture diverse themes, e.g.\ traveling, shopping, etc.
%For each image collection $i$, hundreds of human generated summaries were collected. We heuristically prune the original human summaries using the technique proposed in~\cite{tschiatschek2014learning}. The remaining human summaries $\mathcal{H}^{(i)} = \{H^{(i)}_1, \ldots, H^{(i)}_{N_i} \}$ are considered as approximate maximizers of an unknown function $f(S \mid \groundset_i)$ that we want to learn.
%
%\noindent {\bfseries Evaluation, model, training. }
%We follow the evaluation from~\cite{tschiatschek2014learning,dolhansky2016deep}.
%That is, we train our model on 13 of the 14 image collections and test the model on the held out image collection.
%We report the average VROUGE score~\cite{tschiatschek2014learning} on the hold out image collection.
%The VROUGE score quantifies the quality of a summary for an image collection, capturing notions of coverage and diversity.
%
%\noindent We train a model using the visual features computed in~\cite{tschiatschek2014learning}, similar as in~\cite{dolhansky2016deep}. 
%Our model processes the 628 dimensional feature vector of each image $i$ by first compressing them into 100 dimensional vectors $h_i$ by a fully connected layer with ReLU activations. From this intermediate representation we compute a quality score $q_i$ for every image $i$ by another fully connected layer. From the intermediate representation we also compute means, maxes and variances across the images for every feature. These quantities are transformed into a threshold vector $b$ through another fully connected layer with ReLU activation ($b$ is 100 dimensional as the intermediate representation). The qualities, the threshold vector and intermediate representations parameterize a set function $f(S)=\sum_{i \in S} q_i + \sum_{j=1}^{100} \min(b_i, \sum_{i\in S} h_{i,j})$. We use dropout to avoid overfitting.
%
%\noindent We optimize the likelihood induced by our proposed \greedy Algorithm, using a temperature of $t=1$ and randomly sampled permutations of the items in the training samples (all human generated summaries consist of 10 images and hence computing the exact likelihood according to~\eqref{eq:ll-greedy} is infeasible). For optimization, we used Adam~\cite{kingma2014adam} with a learning rate of $0.001$ and weight decay $0.01$. We performed 20 passes through the training data.
%
%\noindent {\bfseries Results.} 
%We achieve an average normalized VROUGE score of 0.87. This is similar to the performance achieved in~\cite{dolhansky2016deep}. The authors in~\cite{tschiatschek2014learning} achieved an average VROUGE score of 1.13 for their best model by learning a mixture of more than 500 hand specified component functions. In our experiments, we observed that our model easily overfits the training data. So more elaborate regularization methods could potentially improve the performance of our model further.
%
%%Average performance of 0.92 (about the same as Jeff's). Performance of mixtures about 1.14. 
%%More a generalization issue (easy to overfit a CNN). Working on BOWs works better.
%
%% \includegraphics[width=5cm]{images/completion_lowres}
%
%%\subsection{Object detection}
%%
%%For the object detection task, we learn the set function on PASCAL VOC 2007 dataset~\cite{pascal2007}. In this dataset, there are 5000 examples for training and validation and 5000 examples for testing with 20 categories. The output of the Faster R-CNN object detector~\cite{fasterrcnn}, namely the class probabilities and bounding boxes, is used as input for our training procedure. In order to refine candidate bounding boxes, we first use the nonmonotone submodular function 
%%\begin{equation*}
%%f(S) = \sum_{i \in S} u_i - \lambda \sum_{i \in S} \sum_{j \in S} s_{ij}
%%\end{equation*}
%%where $u_i$ corresponds to the class probabilities and $s_{ij}$ corresponds to the Jaccard index of the bounding boxes. Here, $\lambda$ is the parameter which controls the number of bounding boxes to be selected. 
%%
%%However this function is not capable of modeling the inter-class dependencies. For example, the probability of co-occurrence of airplane and dog is quite low, given the nature of the PASCAL dataset. To overcome this, we multiply the Jaccard index matrix of selected bounding boxes with a inter-class similarity matrix which we are going to learn. Since the dataset has 20 classes, the inter-class similarity matrix will be $20$ by $20$. Then we can define the new objective function as
%%\begin{equation*}
%%f(S, W) = \sum_{i \in S} u_i - \lambda \sum_{i \in S} \sum_{j \in S} s_{ij} * w_{ij}
%%\end{equation*}
%%where we learn $w_{ij}$. 
%%\begin{figure}[H]
%%	\centering
%%	\begin{subfigure}[t]{0.45\columnwidth}
%%		\centering
%%		\includegraphics[width=\textwidth]{learned_matrix_greedy.png} 
%%		\subcaption{Learned Similarity Matrix}
%%	\end{subfigure}\hspace{2mm}
%%	\begin{subfigure}[t]{0.45\columnwidth}
%%		\centering
%%		\includegraphics[width=\textwidth]{emp_sim.png}
%%		\subcaption{Empirical Similarity Matrix}
%%	\end{subfigure}
%%\end{figure}
%%We initialize the entries of the matrix $\mathbf{W}$ to 0.1 and in the end, we can see that the learned similarity matrix manages to capture the dependencies similar to empirical similarity matrix. 
%%\
